Reachability Problem for Weak Multi-Pushdown Automata

This paper is about reachability analysis in a restricted subclass of multi-pushdown automata. We assume that the control states of an automaton are partially ordered, and all transitions of an automaton go downwards with respect to the order. We prove decidability of the reachability problem, and computability of the backward reachability set. As the main contribution, we identify relevant subclasses where the reachability problem becomes NP-complete. This matches the complexity of the same problem for communication-free vector addition systems, a special case of stateless multi-pushdown automata.

==> prelim.tex <==
\section{Multi-pushdown automata}
\label{sec:prelim}

A multi-pushdown automaton (\MPDA) is like a single-pushdown one.
In a single step one symbol is popped from one of stacks\footnote{If we allowed for popping from more than one stack at a time,
the model would clearly become Turing-complete, even with one state only.}, and a number of symbols are
pushed on the stacks. 
Assume there are $k$ stacks. A transition of an automaton is thus of the form:
\begin{align} \label{eq:mpdatran}
q, \ \s{X} \ \trans[a] \ q', \ \a_1, \ldots, \a_k,
\end{align}
to mean that when an automaton reads $a$ in state $q$, it pops $\s{X}$ from one of the stacks, pushes the 
sequence of symbols $\a_i$ on the $i$th stack, for $i = 1 \ldots k$, and goes to state $q'$. 
We allow for silent transitions with $a = \eps$.
Observe that wlog. one may assume that stack alphabets are disjoint. 

Formally, the ingredients of an \MPDA\ are: a finite set of states $\al{Q}$,
% together with a distinguished initial state, 
the number of stacks $k$, pairwise-disjoint
finite stack alphabets $\al{S_1} \ldots \al{S_k}$, an input alphabet $\al{A}$, and a finite set
of transition rules:
\begin{equation} \label{eq:transrel}
\trans[] \ \ \subseteq \ \al{Q} \times (\bigcup_{i \leq k} \al{S_i}) \times (\al{A} \cup \{\eps\}) 
\times \al{Q} \times {\al{S_1}}^* \times \ldots \times {\al{S_k}}^*
\end{equation}
written as in~\eqref{eq:mpdatran}.
A configuration of an \MPDA\ is a tuple $\config{q}{\b_1}{\ldots}{\b_k} \in \al{Q} \times \al{S_1}^* \times \ldots \times \al{S_k}^*$.
The transition rules~\eqref{eq:mpdatran} induce the transition relation over all configurations in a standard way:
\[
\frac{q, \ \s{X} \ \trans[a] \ q', \ \a_1, \ldots, \a_k \ \ \ \ \ \ \ \s{X} \in \al{S_i} \ \ \ \ \ \ \ \b_i = \s{X} \b}
{\config{q}{\b_1}{\ldots \b_i \ldots}{\b_k} \trans[a] \config{q'}{\a_1 \b_1}{\ldots \a_i \b \ldots}{\a_k \b_k}}
\]
thus defining the configuration graph of an \MPDA.
For a configuration $\config{q}{\a_1}{\ldots}{\a_k}$, its \emph{size} is defined as 
the sum of lengths of the words $\a_i$, $i \leq k$.
The same applies to a right-hand side of any transition rule $q \ \s{X} \ \trans[a] \ q' \ \a_1 \ldots \a_k$.


An \MPDA\ is \emph{\stateless} if there is just one state (or equivalently no states).
Transition rules of an automaton are then of the form:
\begin{equation} \label{eq:statelessmpdatran}
\s{X} \ \trans[a] \ \a_1, \ldots, \a_k
\end{equation}
and configurations are of the form $\confless{\b_1}{\ldots}{\b_k}$. 

A less severe restriction on control states is the following one.
We say that an automaton is \emph{weak} if there is a partial order $\leq$ on its states 
such that every transition~\eqref{eq:mpdatran} satisfies $q'\leq q$. 
Clearly, every \stateless\ automaton is weak.

\begin{remark}
Note that \stateless\ one-stack automata are essentially context-free grammars in
Grei\-bach normal form. Thus the configuration graphs are precisely context-free graphs,
called also BPA graphs~\cite{PRS,handbook}.
Another special case is many stacks with singleton alphabets. The stacks are thus essentially
counters without zero tests. In this subclass, \stateless\ automata corresponds to communication-free Petri nets~\cite{E97},
called also BPP~\cite{ChrPhd}, or commutative context-free graphs~\cite{CFL11}.
The BPA and BPP classes are members of the Process Rewrite Systems hierarchy of~\cite{PRS} that contains,
among the others, unrestricted pushdown systems and Petri nets.
\end{remark}

\begin{myexample}
\label{ex:automaton}
Assuming a distinguished initial state and acceptance by all stacks empty,
\weak\  \MPDA s\ can recognize non-context-free languages. 
For instance, the language 
\begin{align} \label{eq:langex}
\{ a^n b^n c^n : n \geq 0 \}
\end{align}
is recognized by an automaton described below.
The automaton has two states $q_1,q_2$ and two stacks. The alphabets of the stacks are $\{\s{X},\s{B}, \s{D}\}$ and $\{\s{C}\}$, respectively. 
% moreover there are three terminal symbols $\{a,b,c\}.$
The starting configuration is $(q_1, \s{X}\s{D}, \varepsilon)$.
% and the automaton accepts by a configuration $(q2, \varepsilon , \varepsilon).$
Besides the transition rules, we also present the automaton in a diagram, 
using \emph{push} and \emph{pop} operations with natural meaning.

\begin{minipage}{.55\linewidth}
%\begin{center}
                \begin{tikzpicture}    % [every text node part/.style={align=center}]                
	    	   \node (q1) at (0,0){$q_1$};
	    	   \node (q2) at (4, 0) {$q_2$};
	   	 
                    \path[->] (q1) edge [loop above] node [text width=1cm] {$a,\ pop\ \s{X} $ \\ $push\ \s{X}\s{B},\s{C}$} (q1);
		    \path[->] (q1) edge [loop left] node [text width=1cm] {$\varepsilon,$\\$pop\ \s{X} $} (q1);
		    \path[->] (q1) edge [loop below] node [text width=1cm] {$b,\ pop\ \s{B} $} (q1);
		    \path[->] (q2) edge [loop above] node [text width=1cm] {$c,\ pop\ \s{C} $} (q2);
		    \path[->] (q1) edge  node [above, text width=1cm] {$\varepsilon,\ pop\ \s{D} $} (q2);
               \end{tikzpicture}
%        \end{center}
\end{minipage}
\begin{minipage}{.45\linewidth}
\begin{align*}
q_1, \ \s{X}  \ & \trans[a] \  q_1, \ \s{X}\s{B}, \ \s{C}  \\
q_1, \ \s{X}  \ & \trans[\varepsilon] \  q_1, \ \varepsilon, \ \varepsilon  \\
q_1, \ \s{B}  \ & \trans[b]  \  q_1, \ \varepsilon, \ \varepsilon  \\
q_1, \ \s{D}  \ & \trans[\varepsilon]  \  q_2, \ \varepsilon, \ \varepsilon  \\
q_2, \ \s{C}  \ & \trans[c]  \  q_2, \ \varepsilon, \ \varepsilon 
\end{align*}
\end{minipage}
\ \\

\noindent
The automaton is weak and uses $\varepsilon$-transitions, which may be however easily eliminated.
Acceptance by empty stacks may be easily simulated using acceptance by states.
The language~\eqref{eq:langex} is not recognized by a \stateless\ automaton, as shown in~\cite{CL12}.
\end{myexample}

\begin{myexample}
%\label{ex:automaton}
Non-context-free languages are recognized even by \stateless\ \MPDAs\ with singleton stack alphabets.
%
The class of languages recognized by this subclass is called \emph{commutative context-free} languages~\cite{H83}, 
see also~\cite{CL12}.
One example is the commutative closure of the language of the previous example: the set of all words
with the same number of occurrences  of $a$, $b$ and $c$. 


\end{myexample}
\ \\
In the sequel we do not care about initial states nor about acceptance condition, as we will focus
on the configuration graph of an automaton. Furthermore, as we only consider reachability problems,
the labeling of transitions with input alphabet letters 
will be irrelevant, thus we write $\trans$ instead of $\trans[a]$ from now on. 

Using a standard terminology, we say that an \MPDA\ is \emph{\normed}
if for any state $q$ and any configuration $\config{q}{\a_1}{\ldots}{\a_k}$, 
there is a path to the empty configuration
\[
\config{q}{\a_1}{\ldots}{\a_k} \trans \ldots \trans \config{p}{\eps}{\ldots}{\eps}
\]
for some state $p$.
In general, whenever an \MPDA\ is not assumed to be \normed\ we call it \emph{\unnormed} for clarity.
Note that in all examples above the automata were \normed. In fact \normedness\ is not a restriction as far as languages
are considered.
 In the sequel we will however analyze the configuration graphs, and then \normedness\ will play a role.

Further, we say that an \MPDA\ is \emph{\strnormed}
if for any state $q$ and any configuration $\config{q}{\a_1}{\ldots}{\a_k}$, 
there is a path to the empty configuration
\[
\config{q}{\a_1}{\ldots}{\a_k} \trans \ldots \trans \config{q}{\eps}{\ldots}{\eps}
\]
containing only transitions that do not change state.
Intuitively, whatever is the state $q$ we start in, any top-most symbol $\s{X}$ in any stack may ,,disappear''.
For \stateless\ automata, \strnormedness\ is the same as \normedness.



